ObVi-SLAM: Long-Term Object-Visual SLAM

Robots responsible for tasks over long time scales must be able to localize consistently and scalably amid geometric, viewpoint, and appearance changes. Existing visual SLAM approaches rely on low-level feature descriptors that are not robust to such environmental changes and result in large map sizes that scale poorly over long-term deployments. In contrast, object detections are robust to environmental variations and lead to more compact representations, but most object-based SLAM systems target short-term indoor deployments with close objects. In this paper, we introduce ObVi-SLAM to overcome these challenges by leveraging the best of both approaches. ObVi-SLAM uses low-level visual features for high-quality short-term visual odometry; and to ensure global, long-term consistency, ObVi-SLAM builds an uncertainty-aware long-term map of persistent objects and updates it after every deployment. By evaluating ObVi-SLAM on data from 16 deployment sessions spanning different weather and lighting conditions, we empirically show that ObVi-SLAM generates accurate localization estimates consistent over long-time scales in spite of varying appearance conditions.

==> factor_graph.tex <==
% Using https://github.com/jluttine/tikz-bayesnet

\begin{figure}[tbp]
    \centering

    \resizebox{0.7 \columnwidth}{!}{

\begin{tikzpicture}


\def \ltmcolor {magenta}
\def \shapepriorcolor {violet}
\def \vocolor {blue}
\def \constcolor {red}
\def \objobscolor {orange}
\def \vfobscolor {Green}
\def \minnodesize {0.85cm}

\def \reprojerrshape {rectangle}
\def \ltmshape {circle}
\def \shapepriorshape {regular polygon}
\def \bberrshape {diamond}
\def \voshape {star}


\node[latent, minimum size=\minnodesize](xi) {$x_t$};

\node[latent, right=of xi,  minimum size=\minnodesize](xip1) {$x_{t+1}$};
\node[latent, right=of xip1, minimum size=\minnodesize](xip2) {$x_{t+2}$};


% \factor[left=of xi, \constcolor] {const} {} {} {};
% \factoredge[\constcolor] {xi} {const} {};

\factor[white, left=of xi] {voimin1} {} {} {};
\factoredge[dashed, \vocolor] {xi} {voimin1} {};

\factor[right=of xi, \vocolor, \voshape] {voi} {} {} {};
\factoredge[dashed, \vocolor] {xip1} {voi} {};
\factoredge[dashed, \vocolor] {xi} {voi} {};

\factor[right=of xip1, \vocolor, \voshape] {voip1} {} {} {};
\factoredge[dashed, \vocolor] {xip1} {voip1} {};
\factoredge[dashed, \vocolor] {xip2} {voip1} {};

\factor[white, right=of xip2] {voip2} {} {} {};
\factoredge[dashed, \vocolor] {xip2} {voip2} {};


\node[latent, above=of xi, minimum size=\minnodesize](e1) {$Q^*_j$};




\node[latent, above=of xip2, minimum size=\minnodesize](e2) {$Q^*_{j+2}$};


\node[latent, above=of xip1, minimum size=\minnodesize](e3) {$Q^*_{j+1}$};


\node[latent, above=of $(e1.north)!0.5!(e3.north)$, node distance=0.4, minimum size=\minnodesize, rectangle](ltm) {$LTM^{i-1}$};




\node[draw,\ltmshape ,\ltmcolor, fill=\ltmcolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (ltm_factor1) at ($(ltm)!0.5!(e1)$) {};
\factoredge[\ltmcolor] {e1} {ltm_factor1} {};
\factoredge[,\ltmcolor] {ltm} {ltm_factor1} {};


\node[draw,\ltmshape ,\ltmcolor, fill=\ltmcolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (ltm_factor2) at ($(ltm)!0.5!(e3)$) {};
\factoredge[\ltmcolor] {e3} {ltm_factor2} {};
\factoredge[\ltmcolor] {ltm} {ltm_factor2} {};

\factor[left=0.85 cm of ltm_factor1, \shapepriorcolor, \shapepriorshape] {shape1} {} {} {};
\factoredge[\shapepriorcolor] {e1} {shape1} {};

\factor[right=0.85 cm of ltm_factor2, \shapepriorcolor, \shapepriorshape] {shape3} {} {} {};
\factoredge[\shapepriorcolor] {e3} {shape3} {};

\factor[right=2.65 cm of ltm_factor2, \shapepriorcolor, \shapepriorshape] {shape2} {} {} {};
\factoredge[\shapepriorcolor] {e2} {shape2} {};


\node[draw,\bberrshape,\objobscolor, fill=\objobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (e1x1obs) at ($(xi)!0.5!(e1)$) {};
% \factor[\objobscolor, above=of xi]{e1x1obs} {} {} {}; 
\factoredge[\objobscolor] {e1} {e1x1obs} {};
\factoredge[\objobscolor] {xi} {e1x1obs} {};

% \factor[\objobscolor, above left=of xip1]{e1x2obs} {} {} {}; 
\node[draw,\bberrshape,\objobscolor, fill=\objobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (e1x2obs) at ($(xip1)!0.5!(e1)$) {};
\factoredge[\objobscolor] {e1} {e1x2obs} {};
\factoredge[\objobscolor] {xip1} {e1x2obs} {};

% \factor[\objobscolor, above right=of xip1]{e2x2obs} {} {} {}; 
\node[draw,\bberrshape,\objobscolor, fill=\objobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (e2x2obs) at ($(xip1)!0.5!(e2)$) {};
\factoredge[\objobscolor] {e2} {e2x2obs} {};
\factoredge[\objobscolor] {xip1} {e2x2obs} {};

% \factor[\objobscolor, above left=of xip2]{e1x3obs} {} {} {}; 
\node[draw,\bberrshape,\objobscolor, fill=\objobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (e1x3obs) at ($(xip2)!0.5!(e1)$) {};
\factoredge[\objobscolor] {e1} {e1x3obs} {};
\factoredge[\objobscolor] {xip2} {e1x3obs} {};

% \factor[\objobscolor, above=of xip2]{e2x3obs} {} {} {}; 
\node[draw,\bberrshape,\objobscolor, fill=\objobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (e2x3obs) at ($(xip2)!0.5!(e2)$) {};
\factoredge[\objobscolor] {e2} {e2x3obs} {};
\factoredge[\objobscolor] {xip2} {e2x3obs} {};


\node[draw,\bberrshape,\objobscolor, fill=\objobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (e3x1obs) at ($(xi)!0.5!(e3)$) {};
\factoredge[\objobscolor] {e3} {e3x1obs} {};
\factoredge[\objobscolor] {xi} {e3x1obs} {};

\node[draw,\bberrshape,\objobscolor, fill=\objobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (e3x3obs) at ($(xip2)!0.5!(e3)$) {};
\factoredge[\objobscolor] {e3} {e3x3obs} {};
\factoredge[\objobscolor] {xip2} {e3x3obs} {};



% \factor[\objobscolor, above left=of xip2]{e1x3obs} {} {} {}; 


\node[latent, below left=of xi, minimum size=\minnodesize](v1) {$v_{k}$};
\node[latent, right=of v1, minimum size=\minnodesize](v2) {$v_{k+1}$};
\node[latent, right=of v2, minimum size=\minnodesize](v3) {$v_{k+2}$};
\node[latent, right=of v3, minimum size=\minnodesize](v4) {$v_{k+3}$};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf1x1obs) at ($(xi)!0.5!(v1)$) {};
\factoredge[dashed,\vfobscolor] {v1} {vf1x1obs} {};
\factoredge[dashed,\vfobscolor] {xi} {vf1x1obs} {};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf1x2obs) at ($(xip1)!0.5!(v1)$) {};
\factoredge[dashed,\vfobscolor] {v1} {vf1x2obs} {};
\factoredge[dashed,\vfobscolor] {xip1} {vf1x2obs} {};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf1x3obs) at ($(xip2)!0.5!(v1)$) {};
\factoredge[dashed,\vfobscolor] {v1} {vf1x3obs} {};
\factoredge[dashed,\vfobscolor] {xip2} {vf1x3obs} {};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf2x1obs) at ($(v2)!0.5!(xi)$) {};
\factoredge[dashed,\vfobscolor] {v2} {vf2x1obs} {};
\factoredge[dashed,\vfobscolor] {xi} {vf2x1obs} {};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf2x2obs) at ($(v2)!0.5!(xip1)$) {};
\factoredge[dashed,\vfobscolor] {v2} {vf2x2obs} {};
\factoredge[dashed,\vfobscolor] {xip1} {vf2x2obs} {};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf2x3obs) at ($(v2)!0.5!(xip2)$) {};
\factoredge[dashed,\vfobscolor] {v2} {vf2x3obs} {};
\factoredge[dashed,\vfobscolor] {xip2} {vf2x3obs} {};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf3x1obs) at ($(v3)!0.5!(xi)$) {};
\factoredge[dashed,\vfobscolor] {v3} {vf3x1obs} {};
\factoredge[dashed,\vfobscolor] {xi} {vf3x1obs} {};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf3x2obs) at ($(v3)!0.5!(xip1)$) {};
\factoredge[dashed,\vfobscolor] {v3} {vf3x2obs} {};
\factoredge[dashed,\vfobscolor] {xip1} {vf3x2obs} {};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf3x3obs) at ($(v3)!0.5!(xip2)$) {};
\factoredge[dashed,\vfobscolor] {v3} {vf3x3obs} {};
\factoredge[dashed,\vfobscolor] {xip2} {vf3x3obs} {};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf4x1obs) at ($(v4)!0.5!(xi)$) {};
\factoredge[dashed,\vfobscolor] {v4} {vf4x1obs} {};
\factoredge[dashed,\vfobscolor] {xi} {vf4x1obs} {};

\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf4x2obs) at ($(v4)!0.5!(xip1)$) {};
\factoredge[dashed,\vfobscolor] {v4} {vf4x2obs} {};
\factoredge[dashed,\vfobscolor] {xip1} {vf4x2obs} {};


\node[draw,\reprojerrshape ,\vfobscolor, fill=\vfobscolor,minimum size=5pt, inner
sep=0pt, node distance=0.4] (vf4x3obs) at ($(v4)!0.5!(xip2)$) {};
\factoredge[dashed,\vfobscolor] {v4} {vf4x3obs} {};
\factoredge[dashed,\vfobscolor] {xip2} {vf4x3obs} {};



\factor[\ltmcolor, \ltmshape, right=1.5 cm of e2]{ltm_ex} {LTM} {} {};


\factor[white, above=of ltm_ex]{filler} {} {} {};
\factor[white, left=of ltm_ex]{ltm_left} {} {} {};
\factor[white, right=of ltm_ex]{ltm_right} {} {} {};
\factoredge[\ltmcolor] {ltm_left} {ltm_ex} {};
\factoredge[\ltmcolor] {ltm_right} {ltm_ex} {};

\factor[\shapepriorcolor, \shapepriorshape, below=0.6cm of ltm_ex]{shape_ex} {Shape Prior} {} {};
\factor[white, left=of shape_ex]{shape_left} {} {} {};
\factor[white, right=of shape_ex]{shape_right} {} {} {};
\factoredge[\shapepriorcolor] {shape_left} {shape_ex} {};
\factoredge[\shapepriorcolor] {shape_right} {shape_ex} {};

\factor[\objobscolor, \bberrshape, below=0.6cm of shape_ex]{obj_obs_ex} {Bounding Box} {} {};
\factor[white, left=of obj_obs_ex]{obj_left} {} {} {};
\factor[white, right=of obj_obs_ex]{obj_right} {} {} {};
\factoredge[\objobscolor] {obj_left} {obj_obs_ex} {};
\factoredge[\objobscolor] {obj_right} {obj_obs_ex} {};

\factor[\vocolor, \voshape, below=0.6cm of obj_obs_ex]{vo_ex} {Visual Odom} {} {};
\factor[white, left=of vo_ex]{vo_left} {} {} {};
\factor[white, right=of vo_ex]{vo_right} {} {} {};
\factoredge[\vocolor, dashed] {vo_left} {vo_ex} {};
\factoredge[\vocolor, dashed] {vo_right} {vo_ex} {};

\factor[\reprojerrshape, \vfobscolor, below=0.6cm of vo_ex]{vf_obs_ex} {Reproj. Err} {} {};
\factor[white, left=of vf_obs_ex]{vf_left} {} {} {};
\factor[white, right=of vf_obs_ex]{vf_right} {} {} {};
\factoredge[\vfobscolor, dashed] {vf_left} {vf_obs_ex} {};
\factoredge[\vfobscolor, dashed] {vf_right} {vf_obs_ex} {};

\plate[inner sep=6.5pt]{legend_plate} {(ltm_ex)(shape_ex)(obj_obs_ex)(vo_ex)(vf_obs_ex)(filler)(ltm_left)(ltm_right)} {};
    
\end{tikzpicture}
}
    \caption{ObVi-SLAM factor graph. Factors with solid lines are present for all optimizations, whereas inclusion of factors with dashed lines is dependent on if the optimization is local or global. \AAA{Maybe: The long-term map factor is only present for objects observed in previous sessions.}}
    \label{fig:obvi_slam_factor_graph}
\end{figure}

==> tikzlibrarybayesnet.code.tex <==
% tikzlibrary.code.tex
%
% Copyright 2010-2011 by Laura Dietz
% Copyright 2012 by Jaakko Luttinen
%
% The MIT License
%
% See LICENSE file for more details.

% Load other libraries
\usetikzlibrary{shapes}
\usetikzlibrary{fit}
\usetikzlibrary{chains}
\usetikzlibrary{arrows}

% Latent node
\tikzstyle{latent} = [circle,fill=white,draw=black,inner sep=1pt,
minimum size=20pt, font=\fontsize{10}{10}\selectfont, node distance=1]
% Observed node
\tikzstyle{obs} = [latent,fill=gray!25]
% Constant node
\tikzstyle{const} = [rectangle, inner sep=0pt, node distance=1]
% Factor node
\tikzstyle{factor} = [rectangle, fill=black,minimum size=5pt, inner
sep=0pt, node distance=0.4]
% Deterministic node
\tikzstyle{det} = [latent, diamond]

% Plate node
\tikzstyle{plate} = [draw, rectangle, rounded corners, fit=#1]
% Invisible wrapper node
\tikzstyle{wrap} = [inner sep=0pt, fit=#1]
% Gate
\tikzstyle{gate} = [draw, rectangle, dashed, fit=#1]

% Caption node
\tikzstyle{caption} = [font=\footnotesize, node distance=0] %
\tikzstyle{plate caption} = [caption, node distance=0, inner sep=0pt,
below left=5pt and 0pt of #1.south east] %
\tikzstyle{factor caption} = [caption] %
\tikzstyle{every label} += [caption] %

%\pgfdeclarelayer{b}
%\pgfdeclarelayer{f}
%\pgfsetlayers{b,main,f}

% \factoredge [options] {inputs} {factors} {outputs}
\newcommand{\factoredge}[4][]{ %
  % Connect all nodes #2 to all nodes #4 via all factors #3.
  \foreach \f in {#3} { %
    \foreach \x in {#2} { %
      \path (\x) edge[-,#1] (\f) ; %
      %\draw[-,#1] (\x) edge[-] (\f) ; %
    } ;
    \foreach \y in {#4} { %
      \path (\f) edge[->, >={triangle 45}, #1] (\y) ; %
      %\draw[->,#1] (\f) -- (\y) ; %
    } ;
  } ;
}

% \edge [options] {inputs} {outputs}
\newcommand{\edge}[3][]{ %
  % Connect all nodes #2 to all nodes #3.
  \foreach \x in {#2} { %
    \foreach \y in {#3} { %
      \path (\x) edge [->, >={triangle 45}, #1] (\y) ;%
      %\draw[->,#1] (\x) -- (\y) ;%
    } ;
  } ;
}

% \factor [options] {name} {caption} {inputs} {outputs}
\newcommand{\factor}[5][]{ %
  % Draw the factor node. Use alias to allow empty names.
  \node[factor, label={[name=#2-caption]#3}, name=#2, #1,
  alias=#2-alias] {} ; %
  % Connect all inputs to outputs via this factor
  \factoredge {#4} {#2-alias} {#5} ; %
}

% \plate [options] {name} {fitlist} {caption}
\newcommand{\plate}[4][]{ %
  \node[wrap=#3] (#2-wrap) {}; %
  \node[plate caption=#2-wrap] (#2-caption) {#4}; %
  \node[plate=(#2-wrap)(#2-caption), #1] (#2) {}; %
}

% \gate [options] {name} {fitlist} {inputs}
\newcommand{\gate}[4][]{ %
  \node[gate=#3, name=#2, #1, alias=#2-alias] {}; %
  \foreach \x in {#4} { %
    \draw [-*,thick] (\x) -- (#2-alias); %
  } ;%
}

% \vgate {name} {fitlist-left} {caption-left} {fitlist-right}
% {caption-right} {inputs}
\newcommand{\vgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-left) {}; %
  \node[wrap=#4] (#1-right) {}; %
  % Draw the gate
  \node[gate=(#1-left)(#1-right)] (#1) {}; %
  % Add captions
  \node[caption, below left=of #1.north ] (#1-left-caption)
  {#3}; %
  \node[caption, below right=of #1.north ] (#1-right-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.north) -- (#1.south); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

% \hgate {name} {fitlist-top} {caption-top} {fitlist-bottom}
% {caption-bottom} {inputs}
\newcommand{\hgate}[6]{ %
  % Wrap the left and right parts
  \node[wrap=#2] (#1-top) {}; %
  \node[wrap=#4] (#1-bottom) {}; %
  % Draw the gate
  \node[gate=(#1-top)(#1-bottom)] (#1) {}; %
  % Add captions
  \node[caption, above right=of #1.west ] (#1-top-caption)
  {#3}; %
  \node[caption, below right=of #1.west ] (#1-bottom-caption)
  {#5}; %
  % Draw middle separation
  \draw [-, dashed] (#1.west) -- (#1.east); %
  % Draw inputs
  \foreach \x in {#6} { %
    \draw [-*,thick] (\x) -- (#1); %
  } ;%
}

